Efficient Algorithms with Asymmetric Read and Write Costs

In several emerging technologies for computer memory (main memory), the cost of reading is significantly cheaper than the cost of writing. Such asymmetry in memory costs poses a fundamentally different model from the RAM for algorithm design. In this paper we study lower and upper bounds for various problems under such asymmetric read and write costs. We consider both the case in which all but $O(1)$ memory has asymmetric cost, and the case of a small cache of symmetric memory. We model both cases using the $(M,\omega)$-ARAM, in which there is a small (symmetric) memory of size $M$ and a large unbounded (asymmetric) memory, both random access, and where reading from the large memory has unit cost, but writing has cost $\omega\gg 1$. For FFT and sorting networks we show a lower bound cost of $\Omega(\omega n\log_{\omega M} n)$, which indicates that it is not possible to achieve asymptotic improvements with cheaper reads when $\omega$ is bounded by a polynomial in $M$. Also, there is an asymptotic gap (of $\min(\omega,\log n)/\log(\omega M)$) between the cost of sorting networks and comparison sorting in the model. This contrasts with the RAM, and most other models. We also show a lower bound for computations on an $n\times n$ diamond DAG of $\Omega(\omega n^2/M)$ cost, which indicates no asymptotic improvement is achievable with fast reads. However, we show that for the edit distance problem (and related problems), which would seem to be a diamond DAG, there exists an algorithm with only $O(\omega n^2/(M\min(\omega^{1/3},M^{1/2})))$ cost. To achieve this we make use of a "path sketch" technique that is forbidden in a strict DAG computation. Finally, we show several interesting upper bounds for shortest path problems, minimum spanning trees, and other problems. A common theme in many of the upper bounds is to have redundant computation to tradeoff between reads and writes.

==> DP.tex <==
\section{Dynamic programming problems}

The computation of a DP problem can be view as a DAG, and each node receives the value from the nodes that have edges pointing to this node, and contains some local calculations.

To reduce writes of an algorithm without increasing the computational complexity, we refer to the previous model introduced in Section~\ref{sec:lowerbound}: the computation is to divided into blocks that each can be kept and computed in the fast memory, which is equivalent to partition the DAG into some subcomponents.
Our goal is to find such decomposition that minimizes the overall number of vertices in all blocks that have outgoing edges.

We categorize DP functions into two types. 
The first type of functions has DAG with fixed structure, for example, the functions of edit distance, longest common sequence, minimum matrix multiplication, Floyd-Warshall algorithm, etc. 
The edges of the second type of functions are decided by input data. 
For example, in the knapsack problem, each state in round $i$ has an incoming edge from a certain state in previous round based on the size of the $i$-th object, and the size can be arbitrary, decided by input.
Similar problems include Bellman-Ford algorithm, longest increase sequence, etc. 
In this paper we focus on the first type of DP functions since the partition the graph can be adapted into a variety of problems.
For the problems with the second type of functions, we know the solutions to some specific problems, but they are hard to be generalized.

Also, we limit our scope in this paper into the DP problems that the number of writes and other instructions are in the same order. For example, the minimum matrix multiplication problem needs $O(n^3)$ reads and $O(n^2)$ writes, so that the cost of a straightforward implementation is optimal as $O(n^3)$, and not affected by write efficiency. 
This means that on average, the nodes on the computational DAG of these problems only have constant number of in- and out-degree.

\hide{

\subsection{Floyd--Warshall algorithm algorithm: an example for constant in-degree DAG}

The Floyd--Warshall algorithm was published in its currently recognized form by Robert Floyd in 1962. The main idea is dynamic programming. Consider a graph $G$ with vertices $V$ numbered 1 through $n$. Further consider a function $\SP(i, j, k)$ that returns the shortest possible path from $i$ to $j$ using vertices only from the set $\{1,2,\cdots,k\}$ as intermediate points along the way. Now, given this function, the goal is to find the shortest path from each $i$ to each $j$ using only vertices 1 to $k + 1$. This can be achieved by
$$\SP(i,j,k+1)=\min\{\SP(i,j,k),\SP(i,k+1,k)+\SP(k+1,j,k)\}$$
An illustration of the dependency of the states of a graph with 3 vertices in the second round is provided in Figure~\ref{fig:FW}.  The pseudocode of the Floyd--Warshall algorithm is provided in Algorithm~\ref{algo:FW}.

\begin{algorithm}[!tp]
\caption{The Floyd--Warshall algorithm}
\label{algo:FW}
\textbf{Input}: A weighted graph $G=(V,E)$.\\
\textbf{Output}: All-pair-shortest-path matrix $d_{|V|\times|V|}$.\\
    \vspace{-0.5em}
    \begin{algorithmic}[1]
    \STATE {Initialize the distances of all edges $(i,j,\mb{dist}_{i,j})\in E$ to $d_{i,j}$.}
    \FOR {$k\leftarrow 1$ to $|V|$}
    \FOR {$i\leftarrow 1$ to $|V|$}
    \FOR {$j\leftarrow 1$ to $|V|$}
        \STATE {$d_{i,j}\leftarrow \min\{d_{i,j},d_{i,k}+d_{k,j}\}$.}
    \ENDFOR
    \ENDFOR
    \ENDFOR
    \RETURN {$\chi_{\pi}$}
   \end{algorithmic}
%    \vspace{.5em}
\end{algorithm}

\begin{figure}[t]
\centering
\includegraphics[width=.45\linewidth]{figures/Floyd.pdf}
\vspace{-2em}
\caption{To be written.}\label{fig:FW}
\end{figure}

The reason that the third dimension does not need to appear in the code explicitly is because the distance between $i$ and $j$ in the $k$-th round will be available in the $(k+1)$-th round (black edges in Figure~\ref{fig:FW}). Hence, if this dimension is squeezed out, the computation of the Floyd-Warshall algorithm can be viewed as: in each iteration, an outer product of the $k$-th column and $k$-th row is computed and used to update the whole matrix (dependencies are shown in red and black edges in Figure~\ref{fig:FW}). The main observation is that, the element $f_{i,j}$ is updated every round, but the new value is not used unless in the $i$-th or the $j$-th round. Therefore, we use another order to implement the dynamic programming. In the $k$-th iteration, we compute and update only the $k$-th column and $k$-th row in the matrix. At last, all elements are updated. The number of read in this algorithm is exactly the same ($O(N^3)$) as the original algorithm, but the number of writes is only $O(N^2)$.
The pseudocode for the write-optimal version Floyd--Warshall algorithm is shown in Appendix~\ref{app:FW-Code}.


\subsection{Other problems}

Edit distance (LCS or any DP algorithm that a state only has constant incoming edges from ``nearby'' states): $O(n^2/z)$ read/write complexity where $z$ is the size of ``fast'' memory.

Similarly, the egg dropping problem can be solved using $O(n\log p)$ reads and $O((n\log p)/z)$ writes.

Seam carving algorithm and maximum sub-matrix problem can reduce writes by $O(z)$ times.

Knapsack problem: $O(np)$ reads and $O(n)$ writes, where $p$ is the number of items. Observation: once a certain size can be achieved, it can always be achieved.

\subsection{The Stencil algorithm}

The Stencil algorithm does not belong to dynamic programming since there exist no ``decisions'' during the whole process. However, the computational DAG of stencil is very similar to some of the DP problems like edit distance or seam carving, and similar ideas can apply to avoid writes. More specifically, a $d$-dimensional stencil computation on $n^d$ states for $r$ rounds requires $O(rn^d/z^{1/d})$ writes. Since the number of reads requires is $O(rn^d)$, the algorithm is optimal when $z>k^d$, which is easy to achieve when $d$ is 1, 2 or 3.

The write-optimal algorithm only writes the value from $z^{1/d}$-th rounds to the memory. Inside every $z^{1/d}$ rounds, grids with coordinate $(x_1,\cdots,x_d)$ are computed in increasing order of $\sum{x_i}$.

The lower bound can probably be proved by showing that, for each node, the number of ancestor nodes with $r'$ rounds difference is $(2r'+1)^d$, so somehow we need $1/z^{1/d}$ of overall states to be written to the memory.
}
\input{LCS}




==> Dijkstra-.tex <==
\section{Single-Source Shortest Path}
\label{sec:dijkstra}

The single-source shortest path (SSSP) problem takes a connected
weighted graph $G=(V,E)$ and a source vertex $s\in V$, and outputs the
shortest distances $d(s,v)$ from $s$ to every other vertex in $v\in
V$.  For graphs with non-negative edge weights, the most efficient
algorithm is Dijkstra's algorithm~\cite{dijkstra1959}.

In this section we will study (variants of) Dijkstra's algorithm in
the asymmetric setting. We describe and analyze three versions (two
classics and one new variant) of Dijkstra's algorithm, and the best
version can be chosen based on the values of $\memsize$, $\wcost$, the
number of vertices $n=|V|$, and the number of edges $m=|E|$.

\begin{theorem}
\label{thm:Dijkstra}
The SSSP problem on a graph $G=(V,E)$ with non-negative edge weights
can be solved with I/O cost $\displaystyle Q=O\left(\min\left(n
    \left(\wcost + {m\over \memsize}\right), \wcost(m+n\log
    n),m(\wcost+\log n)\right)\right)$ and \work{} $\W=Q+O(n\log n)$.
\end{theorem}

We start with the classical Dijkstra's algorithm\,\cite{dijkstra1959}.
In this algorithm, $\delta(v)$, a tentative upper bound on the
distance, is kept for each vertex $v$ in the graph, and initialized as
$+\infty$ ($0$ for $\delta(s)$).  The algorithm consists of $n-1$
iterations, and the final distances from the source $s$ are stored in
$\delta(\cdot)$.  In each iteration, the algorithm selects the
unvisited vertex $u$ with smallest finite $\delta(u)$, marks it as
\emph{visited}, and uses its outgoing edges to relax (update) all its
neighbors' distances.  A priority queue is required to efficiently
select the unvisited vertex with minimum distance.  Using a Fibonacci
heap~\cite{fredman1987fibonacci}, the \work{} of the algorithm is
$O(m+n\log n)$ in the standard (symmetric) RAM model.  In the
\ourmodel, the costs are $\W=Q=O(\wcost{}(m+n\log n))$ since the
Fibonacci heap requires proportionally as many writes as reads.
Alternatively, using a binary search tree for the priority queue
reduces the number of writes (see Section~\ref{sec:upper-intro}) at
the cost of increasing the number of reads, giving the costs
$Q=\W=O(m\log n+\wcost{}m)$.  These bounds are better when
$m=o(\wcost{}n)$.  Both these variants store the priority queue in
\slowmem, requiring at least one write to \slowmem{} per edge.

We now describe an algorithm, which we refer to as \emph{phased
  Dijkstra}, that fully maintains the priority queue in \fastmem{}
and only requires $O(n)$ writes to \slowmem{}.  The idea is to
partition the computation into phases such that in each phase the
priority queue fits in \fastmem.  In particular let $\memsize' =
\memsize/c$ (for a small constant $c$), then each phase will maintain
a priority queue of size at most $2\memsize'$ and visit at least
$\memsize'$ vertices.  The only writes in the algorithm to \slowmem{}
are the shortest distances to each vertex.

Each phase starts and ends with an empty priority queue $P$ and
consists of two parts.  The first part loops over all the edges in the
graph and for any edge that goes from a visited vertex to an unvisited
vertex, inserts it into $P$ if not in there, or does a decrease-key if
in there with a larger distance (we use a Fibonacci heap for $P$).
The second part then runs standard Dijkstra's algorithm until $P$ is
empty.  For both parts $P$ is kept small by deleting the $\memsize'$
largest elements (vertex distances) whenever $|P| = 2\memsize'$.  To
do this $P$ is flattened into an array, the $\memsize'$-th smallest
element is found by selection, and the Fibonacci heap is reconstructed
from the elements less than it, all taking linear time.  Also, to
implement relax the algorithm needs to know whether a vertex is
already in $P$ and if so where so it can do a decrease-key on it.  We
cannot afford to store this information with the vertex in \slowmem{},
but it can be stored in \fastmem{} using a hash table.  The
correctness of this phased Dijkstra's follows from the fact that it
only ever visits the closest unvisited vertex, as with standard
Dijkstra's.

\begin{lemma}
  Phased Dijkstra's has I/O cost $\displaystyle
  Q=O\left(n\left({m\over\memsize}+\wcost{}\right)\right)$ and \work{}
  $\W=Q+O(n\log n)$ both in expectation (for $M \leq n$).
\end{lemma}

\begin{proof}
During a phase either the size of $P$ will grow to $2\memsize'$ (and
hence delete some entries) or it will finish the algorithm.  If $P$
grows to $2\memsize'$ then at least $\memsize'$ vertices are visited
during the phase since that many need to be deleted with delete-min to
empty $P$.  Therefore the number of phases is at most $\lceil
n/\memsize'\rceil$.  Visiting all edges in the first part of each
phase involves at most $m$ insertions and decrease-keys into $P$, each
taking $O(1)$ amortized time in \fastmem, and $O(1)$ time to read the
edge from \slowmem.  Since compacting $P$ when it overflows takes
linear time, its cost can be amortized against the insertions that
caused the overflow.  The cost across all phases for the first part is
therefore $Q = W = O(m \lceil n / \memsize' \rceil)$.  For the second
part, every vertex is visited once and every edge relaxed at most once
across all phases.  Visiting a vertex requires a delete-min in
\fastmem{} and a write to \slowmem, while relaxing an edge requires an
insert or decrease-key in \fastmem, and $O(1)$ reads from \slowmem{}.
We therefore have for this second part (across all phases) that $Q =
O(\wcost n + m)$ and $W = O(n(\wcost + \log n) + m)$.  The operations
on $P$ each include an expected $O(1)$ cost for the hash table
operations.  Together this gives our bounds.
\end{proof}

\hide{
%\julian{what is this sentence for?} \yan{This is what we discussed with Jeremy last time. The problem is, if the Fib heap has a size of $M$, then it is not going to fit into a memory with size of $M$ words, because for each heap node, we need at least to store vertex label, distance, and 2 pointers to keep the structure. Thus the size of the heap doesn't match the size of the fast memory. Maybe tomorrow we can discuss about this.} In practice we can set $M'$ to be $M/28$ to allow for some extra
%storage to maintain the data structure in the algorithm.
%% This
%% does not affect the bounds asymptotically.


The pseudocode of the algorithm is provided in
Algorithm~\ref{algo:wo-dijkstra}.
%We now explain the write-optimal Dijkstra's algorithm.
The algorithm is divided into at most $\lceil n/\memsize'\rceil$
\emph{phases}, where the beginning of a phase is when the algorithm
executes Lines 5--9, looping over all of the edges in the graph, and
the phase lasts until just either right before the algorithm executes
Lines 5--9 again, or all vertices have been visited.
A priority queue is used $P$ to keep up to $\memsize'$ unvisited vertices that
are tentatively closest to the source vertex $s$.  Let $P_{\smb{max}}$
be the largest distance of the vertex in $P$ if $P$ contains
$\memsize'$ vertices, and $+\infty$ otherwise.  Then in Lines 10--20,
we run the standard procedure for Dijkstra's algorithm, except that
only the vertices with distances less than $P_{\smb{max}}$ are
relaxed.  More specifically, the distance of a vertex is updated in
the priority queue (insertion if the vertex is not in $P$, and
decrease-key otherwise) if and only if the distance is less than
$P_{\smb{max}}$.
%This is required due to the shortest distance property.
To insert a vertex when $P$ is full, we have to delete the vertex in $P$ with
largest tentative distance to create space, and this process is explained later.
We consider only vertices
with tentative distance less than $P_{\smb{max}}$ to guarantee that all vertices that have closer tentative distances are guaranteed to be in $P$.
%we never remove one of the actual closest $\memsize'$ unvisited vertices
%from the queue.
%% Once the size of $P$ reaches $2\memsize'$, we apply a lazy deletion process
%% that will be discussed later, and reset $P_{\smb{max}}$.
When the priority queue becomes empty, which means that all vertices
with distances less than $P_{\smb{max}}$ are correctly computed, this
phase finishes and a new phase will start.

%% The algorithm needs to maintain a priority queue $P$ in \fastmem{} that effectively stores the $\memsize'$ closest vertices to $s$.
%The algorithm requires a priority queue $P$ in fast memory with size $2\memsize'$.
%In our algorithm, we implement it based on a Fibonacci Heap.
To implement the priority queue, we use a Fibonacci heap, which allows
insertions and decrease-keys to be done in $O(1)$ \work, and
delete-mins in $O(\log \memsize')$ \work.
%% However, the problem is that in a given phase we can encounter a vertex $v \not\in P$ such that its relaxed distance is less than $P_{\smb{max}}$. In such a case we need to delete the vertex in $P$ with largest distance and then insert $v$ into $P$.
However, the standard Fibonnaci heap does not support efficiently
finding and deleting the vertex with maximum distance, an operation
that our algorithm requires.
%% The problem is that the size of the priority queue $P$ can grow in one phase, and the classic version has no effective way to find and delete the vertex with the maximum distances.
%However, when an insertion comes and $P$ is full, the maximum element should be ejected, since $P$ needs to be kept in the fast memory.
%This causes the problem that a regular Fibonacci Heap does not support query-max.
To solve this problem, we modify the Fibonacci heap so that the
deletions are gathered and processed ``lazily''.  The deletions are
delayed until the number of elements in $P$ increases by a constant
factor (say $\memsize'$ deletions are gathered).  Then we flatten $P$
into an array, use quick-selection to find the $\memsize'$-th element,
reconstruct a Fibonacci heap from the first $\memsize'$ elements
%% (a
%% binomial heap initially)
and remove the remaining elements.  It is easy to see that this
process takes $O(\memsize')$ \work, and thus the amortized cost for
each deletion is $O(1)$.
In Line~\ref{check}, we need a hash table to track whether a vertex is in $P$ or not.
If so, the pointer of the heap vertex is given, and we can apply decrease-key to that heap vertex.
\hide{\julian{I don't see why a hash table is
  needed to keep the mapping of vertices. Can we just do the
  decrease-key even if the vertex is not one of the $\memsize'$
  smallest elements? This is effective what deleting it and
  reinserting it is doing.}
  \yan{This is because when we do decrease-key of a vertex, we need to first know where the vertex is in $P$. I guess you want to say is that to use insertion but not decrease-key? Otherwise, I don't think we can decrease a key that does not exist in $P$. If we use insertion, then we might keep duplications of a vertex. Our new Fib heap does not support deletion of an arbitrary element. Even we can do it, we still need to know where it is, which requires the hash table.}}
%% The priority queue $P$ has
%% a maximum size of $2\memsize'$ although only the smallest $\memsize'$
%% elements are valid.  In order to decide whether an element is valid,
%% we use a hash table to keep the mapping of vertices and indices, so
%% that each lookup only requires constant in-memory \work{}.

\begin{algorithm}[t]
\caption{Write-optimal Dijkstra's algorithm}
\label{algo:wo-dijkstra}

    \KwIn{A connected weighted graph $G=(V,E)$ and a source vertex $s$}
    \KwOut{The shortest distances $\delta=\{\delta_1,\ldots, \delta_n\}$ from source $s$}
    \vspace{0.5em}

{Priority Queue $P\leftarrow \varnothing$}\\
{Mark vertex $s$ as visited and set $\delta(s)\leftarrow 0$}\\
\While {there exists unvisited vertices} {
\If {$P = \varnothing$} {
    {Scan over all edges in $E$ and store at most $\memsize'$ closest unvisited vertices in $P$} \label{line1}\\
    \If {$|P|=\memsize'$} {
        {Set $P_{\smb{max}}$ as the distance to the farthest vertex in $P$}
    }
        \Else {$P_{\smb{max}}\leftarrow +\infty$\label{line2}}
    }
{$u=P.\mb{deleteMin}()$ \label{line3}}\\
{Set $\delta_u$ as the distance from $s$ to $u$, and mark $u$ as visited \label{line5}}\\
\ForEach {$(u,v,\mb{dis}_{u,v})\in E$} {
    \If {$\delta_u+\mb{dis}_{u,v}<P_{\smb{max}}$} {
        \If {$v\in P$\label{check}} {
            {$P.\mb{decreaseKey}(v,\delta_u+\mb{dis}_{u,v})$}
        }
        \Else {
            {$P.\mb{insert}(v,\delta_u+\mb{dis}_{u,v})$}\\
            \If {$|P| = 2\memsize'$} {
                {Remove $\memsize'$ vertices with largest distances in $P$}\\
                {Set $P_{\smb{max}}$ as the distance to the farthest vertex in $P$\label{line4}}
            }
        }
    }
}
}
\Return $\delta(\cdot)$
\end{algorithm}


Now we consider the costs $Q$ and $W$ for the algorithm.  The number
of phases is at most $\lceil n/\memsize'\rceil$ since at least
$\memsize'$ vertices are visited in each phase (in fact many more than
$\memsize'$ might be visited, possibly finishing the algorithm in one
phase).
%% We first analyze the number of phases of the algorithm.
%% If the queue is never full (containing less than $\memsize'$ elements), the new algorithm will act the same as the classic Dijkstra's algorithm and terminate in this round.
%% Otherwise, the queue is full in a certain time in this phase and emptied at last, so at least $\memsize'$ vertices are proceeded in this phase, which limits the number of phases to be at most $\lceil n/\memsize'\rceil$.
In each phase, at most $m$ insertions plus decrease-keys are used to
initialized the priority queue (Lines~\ref{line1}--\ref{line2}), and
at most $m$ edges can relax the distances in one phase
(Lines~\ref{line3}--\ref{line4}). These operations are all in
\fastmem{} and the \work{} for each of operations is constant, so the
\work{} is $O(m)$ per phase. The I/O cost is $O(m)$ as each edge is read
once on Line 5 and at most once on Line 12.  Each vertex will be
extracted from the delete-min on Line 10 exactly once throughout the
algorithm, so the total \work{} is $O(n\log\memsize')$.
%% \memsizeeanwhile, for each vertex, one corresponding delete-min is operated in a specific phase.
%% The total cost for delete-min is $O(\log\memsize')$ for each vertex, multiplied by $n$, the number of vertices.
Lastly, there is one write to \slowmem{} per vertex on
Line~\ref{line5} when it is extracted from the delete-min.
 %% the final answer is written to \slowmem{} after the closest vertex is selected in current frontier (Line~\ref{line5}).
Overall, the I/O cost $Q$ is $O((n/\memsize') m+\wcost{}n)$, and the
\work{} $\W$ is $Q+O(n+n\log n)$.

\begin{lemma}
  Algorithm~\ref{algo:wo-dijkstra} has I/O cost $\displaystyle
  Q=O\left(n\left({m\over\memsize}+\wcost{}\right)\right)$ and \work{}
  $\W=Q+O(n\log n)$.
\end{lemma}
}

Comparing to the first two Dijkstra's algorithms with
$Q=\W=O(\wcost{}m+\min(\wcost{}n\log n,m\log n))$, the new algorithm
is strictly better when $\wcost \memsize>n$.
%% For example, for a cache
%% size $\memsize\sim 10^6$ and $\wcost \sim 10^3$ (which is the case for
%% many hardware settings), phased Dijkstra's performs better than the
%% first two algorithms on graphs with a million to a billion vertices.
More specifically, the new algorithm performs better when
$nm/M<\max\{\wcost{}m,\min(\wcost{}n\log n,m\log n)\}$.

\vspace{0.5em}
Combining these three algorithms proves Theorem~\ref{thm:Dijkstra},
when the best one is chosen based on the parameters $\memsize$,
$\wcost$, $n$, and $m$.


%For non-sparse graph that has $\omega(n)$ edges (here $\omega$ is the asymptotic bound not the write cost), we now introduce a new algorithm that solves the SSSP and needs at most $O(n/\memsize\cdot m+n\log n)$ instructions but only $O(n)$ writes.


==> Dijkstra-back.tex <==
\section{Single-Source Shortest Path}
\label{sec:dijkstra}

The single-source shortest path (SSSP) problem takes a connected weighted graph
$G=(V,E)$ and a source vertex $s\in V$, and outputs the shortest distances $d(s,v)$
from $s$ to every other vertex in $v\in V$.
For graphs with non-negative edge weights, the most
efficient algorithm is Dijkstra's algorithm~\cite{dijkstra1959}.

In this section we will study (variants of) Dijkstra's algorithm in
the the asymmetric setting. We describe and analyze three versions
(two classics and one new variant) of Dijkstra's algorithm, and the
best version can be chosen based on the values of $M$, $\wcost$,
the number of vertices $n=|V|$, and the number of edges $m=|E|$.

\begin{theorem}
\label{thm:Dijkstra}
The SSSP problem on a graph $G=(V,E)$ with non-negative edge weights
can be solved with I/O cost $\displaystyle Q=O\left(\min\left(n \left(\wcost + {m\over M}\right),
\wcost(m+n\log n),m(\wcost+\log n)\right)\right)$ and work $W=Q+O(n\log n)$.
\end{theorem}

We start with the classical Dijkstra's algorithm\,\cite{dijkstra1959}.
In this algorithm, $\delta(v)$, a tentative upper bound on the
distance, is kept for each vertex $v$ in the graph, and initialized as
$+\infty$ ($0$ for $\delta(s)$).
The algorithm
consists of $n-1$ iterations, and the final distances from the source $s$ are
stored in $\delta(\cdot)$.
In each iteration, the algorithm
selects the vertex $u$ with smallest finite $\delta(u)$ and mark it as \emph{visited}, and uses its
outgoing edges to relax all its neighbors' distances.

A priority queue is required
to efficiently select of the unvisited vertex with minimum distance.
If we use Fibonacci
heap~\cite{fredman1987fibonacci}, the work of the
algorithm is $O(m+n\log n)$ in the standard (symmetric) RAM model.  In
the asymmetric model, the work and I/O costs are
$Q=W=O(\wcost{}(m+n\log n))$ since each operation corresponds to a
write to the Fibonacci heap, which is stored in slow memory.

Alternatively, we can use balanced binary search tree to maintain the
priority queue, since each insertion and deletion requires an
amortized constant number of writes (see
Section~\ref{sec:upper-intro}).  Therefore, the number of writes are
reduced at the expense of performing more reads.  This algorithm
requires I/O cost and work $Q=W=O(m\log n+\wcost{}m)$, and performs
better than the previous algorithm when $m=o(\wcost{}n)$.

However, both of these methods store the
priority queue in slow memory, which leads to excessive writes.  We now
present a new algorithm that runs Dijkstra's algorithm mostly in fast memory and only writes the final distances to slow memory.
%We refer to this algorithm as \emph{write-optimal Dijkstra's algorithm},
This algorithm only requires $O(n)$ writes to slow memory, which is optimal
in terms of the number writes for the SSSP problem (the output size is
$\Theta(n)$).

The overall idea of the algorithm is to partition the computation into
phases, such that in each phase we only need the size of the priority queue to be $M' \le M$, small enough to
fit in fast memory.  We guarantee that the shortest
distances of at least $\memsize'$ vertices can be computed in each
phase, so the algorithm terminates after at most $\lceil n/\memsize' \rceil$ phases.
The only writes in the algorithm to slow memory are the shortest distances to
each vertex (or the shortest path tree if required).

\julian{what is this sentence for?} \yan{This is what we discussed with Jeremy last time. The problem is, if the Fib heap has a size of $M$, then it is not going to fit into a memory with size of $M$ words, because for each heap node, we need at least to store vertex label, distance, and 2 pointers to keep the structure. Thus the size of the heap doesn't match the size of the fast memory. Maybe tomorrow we can discuss about this.} In practice we can set $M'$ to be $M/28$ to allow for some extra
storage to maintain the data structure in the algorithm.
%% This
%% does not affect the bounds asymptotically.

The pseudocode of
the write-optimal Dijkstra's algorithm is provided in
Algorithm~\ref{algo:wo-dijkstra}.
%We now explain the write-optimal Dijkstra's algorithm.
The algorithm is divided into at most $\lceil n/\memsize'\rceil$
\emph{phases}, where the beginning of a phase is when the algorithm
executes Lines 5--9, looping over all of the edges in the graph, and
the phase lasts until just either right before the algorithm executes
Lines 5--9 again, or all vertices have been visited.  Each phase uses
a priority queue $P$ to keep up to $\memsize'$ unvisited vertices that
are tentatively closest to the source vertex $s$.  Let $P_{\smb{max}}$ be the
largest distance of the vertex in $P$ if $P$ contains $\memsize'$
vertices, and $+\infty$ otherwise.  Then in Lines 10--20, we run the
standard procedure for Dijkstra's algorithm, except that only the
vertices with distances less than $P_{\smb{max}}$ are relaxed.
More specifically, the distance of a vertex is updated in the priority
queue (insertion if the vertex is not in $P$, and decrease-key
otherwise) if and only if the distance is less than $P_{\smb{max}}$.
%This is required due to the shortest distance property.
To insert a vertex we have to first delete the vertex in $P$ with
largest tentative distance to create space.  We consider only vertices
with tentative distance less than $P_{\smb{max}}$ to guarantee that we
never remove one of the actual closest $\memsize'$ unvisited vertices
from the queue.
%% Once the size of $P$ reaches $2M'$, we apply a lazy deletion process
%% that will be discussed later, and reset $P_{\smb{max}}$.
When the
priority queue becomes empty, which means that all vertices with
distances less than $P_{\smb{max}}$ are correctly computed, this phase
finishes and a new phase will start.

%% The algorithm needs to maintain a priority queue $P$ in fast memory that effectively stores the $\memsize'$ closest vertices to $s$.
%The algorithm requires a priority queue $P$ in fast memory with size $2\memsize'$.
%In our algorithm, we implement it based on a Fibonacci Heap.
To implement the priority queue, we
use a Fibonacci heap, which allows insertions and decrease-keys to be done in $O(1)$ time, and delete-mins in $O(\log \memsize')$ time.
%% However, the problem is that in a given phase we can encounter a vertex $v \not\in P$ such that its relaxed distance is less than $P_{\smb{max}}$. In such a case we need to delete the vertex in $P$ with largest distance and then insert $v$ into $P$.
However,
the standard Fibonnaci heap does not support efficiently finding and deleting the vertex with maximum distance, an operation that our algorithm requires.
%% The problem is that the size of the priority queue $P$ can grow in one phase, and the classic version has no effective way to find and delete the vertex with the maximum distances.
%However, when an insertion comes and $P$ is full, the maximum element should be ejected, since $P$ needs to be kept in the fast memory.
%This causes the problem that a regular Fibonacci Heap does not support query-max.
To solve this problem, we modify the Fibonacci heap so that the
deletions are gathered and processed ``lazily''.  The deletions are
delayed until the number of elements in $P$ increases by a constant
factor (say $\memsize'$ deletions are gathered).  Then we flatten $P$
into an array, use quick-selection to find the $\memsize'$-th element,
reconstruct a Fibonacci heap from the first $\memsize'$ elements
%% (a
%% binomial heap initially)
and remove the remaining elements.  It is
easy to see that this process takes $O(\memsize')$ time, and thus the
amortized cost for each deletion is $O(1)$.
\julian{I don't see why a hash table is needed to keep the mapping of vertices. Can we just do the decrease-key even if the vertex is not one of the $\memsize'$ smallest elements? This is effective what deleting it and reinserting it is doing.}
\yan{This is because when we do decrease-key of a vertex, we need to first know where the vertex is in $P$. I guess you want to say is that to use insertion but not decrease-key? Otherwise, I don't think we can decrease a key that does not exist in $P$. If we use insertion, then we might keep duplications of a vertex. Our new Fib heap does not support deletion of an arbitrary element. Even we can do it, we still need to know where it is, which requires the hash table.}
%% The priority queue $P$ has
%% a maximum size of $2\memsize'$ although only the smallest $\memsize'$
%% elements are valid.  In order to decide whether an element is valid,
%% we use a hash table to keep the mapping of vertices and indices, so
%% that each lookup only requires constant in-memory work.

\begin{algorithm}[t]
\caption{Write-optimal Dijkstra's algorithm}
\label{algo:wo-dijkstra}

    \KwIn{A connected weighted graph $G=(V,E)$ and a source vertex $s$}
    \KwOut{The shortest distances $\delta=\{\delta_1,\ldots, \delta_n\}$ from source $s$}
    \vspace{0.5em}

{Priority Queue $P\leftarrow \varnothing$}\\
{Mark vertex $s$ as visited and set $\delta(s)\leftarrow 0$}\\
\While {there exists unvisited vertices} {
\If {$P = \varnothing$} {
    {Scan over all edges in $E$ and store at most $M'$ closest unvisited vertices in $P$} \label{line1}\\
    \If {$|P|=M'$} {
        {Set $P_{\smb{max}}$ as the distance to the farthest vertex in $P$}
    }
        \Else {$P_{\smb{max}}\leftarrow +\infty$\label{line2}}
    }
{$u=P.\mb{deleteMin}()$ \label{line3}}\\
{Set $\delta_u$ as the distance from $s$ to $u$, and mark $u$ as visited \label{line5}}\\
\ForEach {$(u,v,\mb{dis}_{u,v})\in E$} {
    \If {$\delta_u+\mb{dis}_{u,v}<P_{\smb{max}}$} {
        \If {$v\in P$} {
            {$P.\mb{decreaseKey}(v,\delta_u+\mb{dis}_{u,v})$}
        }
        \Else {
            {$P.\mb{insert}(v,\delta_u+\mb{dis}_{u,v})$}\\
            \If {$|P| = 2M'$} {
                {Remove $\memsize'$ vertices with largest distances in $P$}\\
                {Set $P_{\smb{max}}$ as the distance to the farthest vertex in $P$\label{line4}}
            }
        }
    }
}
}
\Return $\delta(\cdot)$
\end{algorithm}

The correctness of this algorithm is easy to see.  Now we show the
upper bound for the I/O cost $Q$ and work $W$ of this algorithm.  The
number of phases is at most $\lceil n/\memsize'\rceil$ since the
shortest distances for at least $\memsize'$ vertices are computed in
each phase.\footnote{Note that if the queue is never full, then there
  will only be a single phase and the algorithm is the same as the
  original Dijkstra's algorithm.}
%% We first analyze the number of phases of the algorithm.
%% If the queue is never full (containing less than $\memsize'$ elements), the new algorithm will act the same as the classic Dijkstra's algorithm and terminate in this round.
%% Otherwise, the queue is full in a certain time in this phase and emptied at last, so at least $\memsize'$ vertices are proceeded in this phase, which limits the number of phases to be at most $\lceil n/\memsize'\rceil$.
In each phase, at most $m$ insertions plus decrease-keys are used to initialized the priority queue (Lines~\ref{line1}--\ref{line2}), and at most $m$ edges can relax the distances in one phase (Lines~\ref{line3}--\ref{line4}). These operations are all in fast memory and the work for each of operations is constant, so the work is $O(m)$ per phase. The I/O cost is $O(m)$ as each edge is read once on Line 5 and at most once on Line 12.
Each vertex will be extracted from the delete-min on Line 10 exactly once throughout the algorithm, so the total work is $O(n\log\memsize')$.
%% Meanwhile, for each vertex, one corresponding delete-min is operated in a specific phase.
%% The total cost for delete-min is $O(\log\memsize')$ for each vertex, multiplied by $n$, the number of vertices.
Lastly, there is one write to slow memory per vertex on Line~\ref{line5} when it is extracted from the delete-min.
 %% the final answer is written to the slow memeory after the closest vertex is selected in current frontier (Line~\ref{line5}).
Overall, the I/O cost $Q$ is $O((n/\memsize') m+\wcost{}n)$, and the work $W$ is $Q+O(n+n\log n)$.

\begin{lemma}
Algorithm~\ref{algo:wo-dijkstra} has I/O cost $\displaystyle Q=O\left(n\left({m\over\memsize}+\wcost{}\right)\right)$ and work $W=Q+O(n\log n)$.
\end{lemma}

Comparing to the first two Dijkstra's algorithms with
$Q=W=O(\wcost{}m+\min(\wcost{}n\log n,m\log n))$, the new algorithm is strictly better
when $\wcost \memsize>n$.
\julian{Don't we also need $nm/M < \min(\wcost n\log n, m\log n)$?} \yan{I changed the previous sentence. Is it more clear now?}
%When $m=o(n\log n)$, the condition changes to $\wcost{}\cdot \memsize>m\log n$.
For example, for a cache size $\memsize\sim 10^6$ and $\wcost \sim 10^3$ (which is the case for many hardware settings), Algorithm~\ref{algo:wo-dijkstra} performs better than the first two algorithms on
graphs with a million to a billion vertices.
%\vspace{0.5em}
Combining these three algorithms proves Theorem~\ref{thm:Dijkstra},
when the best one is chosen based on the parameters $M$, $\wcost$, $n$, and $m$.


%For non-sparse graph that has $\omega(n)$ edges (here $\omega$ is the asymptotic bound not the write cost), we now introduce a new algorithm that solves the SSSP and needs at most $O(n/\memsize\cdot m+n\log n)$ instructions but only $O(n)$ writes.


==> MST-back.tex <==
\section{Minimum Spanning Tree (MST)}
\label{sec:MST}

In this section we discuss several commonly-used algorithms for
computing a minimum spanning tree (MST) on a weighted graph
$G=(V,E)$ with $n=|V|$ vertices and $m=|E|$ edges.  Some of them are
optimal in terms of the number of writes ($O(n)$).  Although loading a
graph into the slow memory requires $O(m)$ writes, these algorithms
are still useful on applications that computes multiple MSTs based on
one input graph.  For example, we can compute different MSTs on
subgraphs (like on road maps).  In some cases, the edge weights can be
described using time-varying functions (e.g., traffic intensity on
electricity networks or road maps changes over time), so it is likely
that the MST algorithms are run multiple times on the same graph
structure.

\myparagraph{Prim's algorithm} All three versions of Dijkstra's
algorithm discussed in Section~\ref{sec:dijkstra} can be adapted to
implement Prim's algorithm~\cite{CLRS}. Thus, the upper bounds of I/O cost and
work in Theorem~\ref{thm:Dijkstra} also hold for minimum spanning
trees.

\myparagraph{Kruskal's algorithm} The initial sorting phase requires
$Q=W=O(m\log n+\wcost{}m)$~\cite{BFGGS15}.  The second phase
constructs a MST using union-find without path compression in $O(m\log
n)$ work, and performs $O(n)$ writes (the actual edges of the
MST). Thus, the complexity is dominated by the first phase.

\myparagraph{Boruvka's algorithm} Boruvka's algorithm consists at most $\log n$ rounds.
Initially all vertices belong in their own component, and
in each round, the lightest edges that connects a component to another component are added to the edge set of the MST, and components are merged using these edges.
Tracking components uses a union-find data structure.
We now introduce an new version of Boruvka's algorithm which is asymptotical optimal of the number of writes.
Here we assume that the edges are stored using adjacency list (either semi-sorted or maintained using a linked list). \julian{why is graph representation discussed here but not in any of the other algorithms?}
\begin{lemma}\label{lemma:boruvka}
The new version of Boruvka's algorithm generates a minimum spanning tree on a graph with $n$ vertices and $m$ edges with I/O cost and work $Q=W=O(m\log n+\wcost{}n)$.
\end{lemma}
%% The new algorithm consists three phases.
For the first $\log \log n$ rounds. we still use union-find to
maintain the connectivity of the component, but without using path
compression and linking two trees in an arbitrary direction.  Thus,
each find operation requires $O(\log\log n)$ time as the height of the
union-find trees is $O(\log\log n)$.  Since there are at most
$2m\log\log n$ queries during the first $\log \log n$ rounds, the
total number of reads is $O(m(\log\log n)^2)$.  The number of writes
is $O(n)$.

After $\log\log n$ rounds, we fully compress paths for all vertices
using $O(n\log\log n)$ reads and $O(n)$ writes. At this point there are at most
$n/\log n$ super-vertices, and from now on, the union-find data structure
is maintained on the super-vertices instead of the original vertices.

We then run the remaining $\log n-\log\log n$ rounds of the algorithm.
Every time two components are merged, we use enforced path compression
(change all the pointers of super-vertices from the smaller-size
components to the root of the larger one). \julian{Is enforced path compression a standard term? Is this union-by-rank?} For a find operation, we
need only two reads (one to find the super-vertex and then one to
follow its parent pointer) to determine its component.  For the union
operation, the parent pointer of each super-vertex is changed at most
$\log n$ times since its component will always be merged into a larger
one and the size at least doubles. The sizes of the components are updated on each union. As there are at most $n/\log n$ super-vertices, the overall
number of writes is $O(n)$. The number of reads per round is $O(m)$,
which gives $O(m\log n)$ reads overall. Summing the I/O cost and work over all rounds of the algorithm proves Lemma~\ref{lemma:boruvka}.


%If the edges of each vertex are sorted by length, the time complexity decreases to $O(m)$.%, and the number of writes increases to $O(\min(m, n\log n))$. (This goes back to the discussion last time: even if we have $n$ processors with local storage space, I don't know how to handle synchronization after each iteration.)



==> fft.tex <==
\section{FFT}

We now consider upper and lower bounds for computations
on an FFT (butterfly) network.

\paragraph{Lower Bounds}

Let $G = (V,E)$ be a directed acyclic graph with vertices $V$ and
edges $E$.  We use $I(G)$ and $O(G)$ to refer to the subsets of
vertices in $G$ with no in-edges and out-edges, respectively.
Consider a collection of subset of $V$, $O = \{O_1, \ldots O_l\}$,
which we will refer to as the \emph{output} sets.  Let $\bar{O} =
\bigcup_{o \in O} o$, and let the predicate $P(v,U)$ be true if there
is a path from $v \in V \setminus U$ to any vertex in $U \subset V$
that does not go through any other vertex in $\bar{O}$.  Each $o \in O$
defines a \emph{cluster} in which the outputs are $o$, and the inputs
are all vertices $v$ in either the DAG inputs $I(G)$ or the cluster
outputs $\bar{O}$ for which $P(v,o)$.

We will refer to $O$ as a $(R,W)$ clustering if the following
properties hold:
\begin{enumerate}
\item each cluster has at most $R$ inputs, i.e., $\forall_{o \in O} |\{v \in I(G) \cup \bar{O}~|~P(v,o)\}| \leq R$ 
\item each cluster has at most $W$ outputs, i.e., $\forall_{o \in O} |o| \leq W$,
\item the cluster outputs cover the DAG outputs, i.e., $O(G) \subseteq \bar{O}$.
\end{enumerate}

Consider a red-black pebbling game~\cite{HK81} on a DAG which each
step consists of one of the following transitions:
\begin{enumerate}
\item (input) A red pebble may be placed on any vertex with a blue pebble.
\item (output) A blue pebble may be placed on any vertex with a red pebble.
\item (compute) A red pebble may be placed on any vertex if every immediate
  predecessor has a red pebble on it.
\item (delete) A pebble (red or blue) may be removed from any vertex.
\end{enumerate}
The DAG starts with a blue pebble on every input, and must end with a
blue pebble on every output.  
We refer to the asymmetric cost of a game $Q$ as the total number
of input steps plus $\omega$ times the number of output steps.

The following theorem relates the pebbling game to our clusters.  In
particular it implies that any lower bound on the number of clusters
implies a lower bound on $Q$.

\begin{theorem}
For a DAG $G$ any red-blue pebbling game with total asymmetry cost $Q$
and using at most $M$ red pebbles corresponds to a $((\omega +1) M,
2M)$ clustering of $G$ with $Q/(\omega M)$ clusters.
\end{theorem}
\begin{proof}
Partition the steps into groups that each have cost $\omega M$
(rounding up).  We show each partition corresponds to a cluster in an
$((\omega +1) M, 2M)$ clustering.  The output set for each cluster
(partition) are all vertices that have taken an output step during the
partition, and all vertices that have a red pebble on them at the end
of the partition (just after the last step of the partition).  There
can be at most $2M$ such vertices.  We now argue that each such
cluster can have at most $(\omega + 1) M$ inputs.  For a cluster
(partition) $o$ the inputs must either correspond to an input step
during the partition or must correspond to a vertex that is red at the
start of the partition. [Needs a bit more description].
\end{proof}

\begin{theorem}
Any $(R,W)$ clustering of an $n$ input FFT DAG has at least
$n \log 2n / (W \log 2R))$ clusters.
\end{theorem}
\begin{proof}
Consider the following accounting scheme for partitioning the unit
weight of each vertex across output vertices in $\bar{O}$.  If a
vertex is an cluster output, then assign the weight to itself.
Otherwise take the weight divide it evenly between the number of
out-edges, and recursively partition this for each corresponding
vertex.  Since each vertex is partitioned, the sum of the weights
assigned across the output vertices exactly equals $|V| = n \log 2n$.
We now argue that every output vertex can have at most $\log 2R$
weight assigned to it.  Looking back from an output vertex we see a
binary tree.  By induction on the tree structure the weight of that
tree is maximized when it is perfectly balanced, which gives a total
weight of $\log 2R$ [needs more proof].  Therefore since every cluster
can have at most $W$ outputs, the total weight assigned to each
cluster is $W \log 2R$.  The number of clusters is therefore at least
$|V| / (W \log 2R)$.
\end{proof}



